TELA: Text to Layer-wise 3D Clothed Human Generation

This paper addresses the task of 3D clothed human generation from textural descriptions. Previous works usually encode the human body and clothes as a holistic model and generate the whole model in a single-stage optimization, which makes them struggle for clothing editing and meanwhile lose fine-grained control over the whole generation process. To solve this, we propose a layer-wise clothed human representation combined with a progressive optimization strategy, which produces clothing-disentangled 3D human models while providing control capacity for the generation process. The basic idea is progressively generating a minimal-clothed human body and layer-wise clothes. During clothing generation, a novel stratified compositional rendering method is proposed to fuse multi-layer human models, and a new loss function is utilized to help decouple the clothing model from the human body. The proposed method achieves high-quality disentanglement, which thereby provides an effective way for 3D garment generation. Extensive experiments demonstrate that our approach achieves state-of-the-art 3D clothed human generation while also supporting cloth editing applications such as virtual try-on. Project page: http://jtdong.com/tela_layer/

==> sec/teaser.tex <==
\begin{center}
\includegraphics[width=1\linewidth]{figures/teaser3.pdf}
\end{center} %\vspace{-53em}
\captionof{figure}{Given textural descriptions (e.g., ``a man wearing jeans, a denim shirt, and a windbreaker''), this paper aims to generate clothing-disentangled 3D human models progressively. Meanwhile, our approach enables high-quality 3D cloth generation and supports applications like cloth transfer.  }
\label{fig:teaser}
